An exact dynamic programming algorithm, lower and upper bounds, applied to the large block sale problem

In this article, we address a class of non convex, integer, non linear mathematical programs using dynamic programming. The mathematical program considered, whose properties are studied in this article, may be used to model the optimal liquidation problem of a single asset portfolio, held in a very large quantity, in a low volatility and perfect memory market, with few market participants. In this context, the Portfolio Manager's selling actions convey information to market participants, which in turn lower bid prices and further penalize the liquidation proceeds we attempt to maximize. We show the problem can be solved exactly using Dynamic Programming (DP) in polynomial time. However, exact resolution is only efficient for small instances. For medium size and large instances, we introduce dedicated heuristics which provide thin admissible solutions, hence tight lower bounds for the initial problem. We also benchmark them against a commercial solver, such as LocalSolver [7]. We are also interested in the continuously relaxed problem, which is non convex. Firstly, we use continuous solutions, obtained by free solver NLopt [26] and transform them into thin admissible solutions of the discrete problem. Secondly, we provide, under some convexity assumptions, an upper bound for the continuous relaxation, and hence for the initial (integer) problem. Numerical experiments confirm the quality of proposed heuristics (lower bounds), which often reach the optimal, or prove very tight, for small and medium size instances, with a very fast CPU time. Our upper bound, however, is not tight.

==> defProblem_VF.tex <==
We consider an investor in a financial market, who holds $N$ units of an asset and wishes to liquidate them over a given time horizon, split in $T$ time steps.\\
He decides to sell at each time step the quantity $x_t \in [\![0;N]\!] $ of a single asset. Hence, the admissible decisions set is defined by:
\begin{equation}
 \DD = \left\{ (x_1,\ldots,x_T)\in \NN^T, \phantom{1} \sum_{t=1}^{T} x_t = N \right\} %= \CC \cap \NN^N
\end{equation}

For each time step $t \in [\![1;T]\!]$, $x_t\geq 0$, we assume a sell only program, and let $p_t>0$ be the asset best bid price.
We also assume there is a minimal floor price $q_t>0$ for very large block trades, with $q_t<p_t$. To simplify notations, we define $c_t = p_t - q_t >0$.
We also introduce a strictly increasing function $g$ from $\NN$ to $[0,1[\;$, such that $g(0)=0$ and $\displaystyle\lim_{+ \infty} g = 1$.\\
At a given time $t$, the execution price of a block of $x_t$ units of asset is modeled by:
\begin{equation}
	v_t(x_t)= p_t\, x_t - (p_t-q_t)\cdot x_t \cdot g\left(\displaystyle\sum_{k=1}^{t} x_k\right) = \left[p_t- c_t\cdot g\Big(\displaystyle\sum_{k=1}^{t} x_k\Big)\right]x_t
\end{equation}
Let f be the objective value function from $\NN^T\rightarrow\RR$:
\begin{equation}
 f(x)=\displaystyle\sum_{t=1}^{T}v_t(x_t)=\displaystyle\sum_{t=1}^{T}\Big[p_t- c_t\cdot g\Big(\displaystyle\sum_{k=1}^{t} x_k\Big)\Big]x_t
\end{equation}
Penalty function $g$ models the market response to the investor selling action, taking into account market memory.
$p_t$ is indeed only valid for a very low traded volume compared to N. Higher volumes lead to lower execution prices, but the pace of decrease reflect market participants information about our intent. The more information, the lower the price. Penalty function $g$ is applied to $y_t=\sum_{k=1}^{t} x_k$, the asset's liquidated quantity up to current time t. $y_t$ represents the available information in a market with perfect memory. Hence, $q_t$ corresponds to the maximum impact, where the market is fully aware of our intentions and react accordingly. The penalty is increasing in $y_t$. The higher $y_t$, the closer the executed price to $q_t$, which justifies our assumptions for $g$.

Therefore, the investor's problem consists of maximizing the sale proceeds from his holding: 
\begin{equation}
	\mbox{OPT} = \displaystyle\max_{x \in \DD} f(x) \label{pbMain0}
\end{equation}

Problem (\ref{pbMain0}) is well defined, as $\DD$ is finite. In the most general case, (\ref{pbMain0}) is an non convex, non separable, non linear, integer optimization problem.\\
  
One will also be interested in the continuous relaxation of the problem. Hence, we extend previous notations.
Let $\CC$ be the set corresponding set of admissible solutions: 
  
\begin{equation}
	\CC = \left\{ (x_1,\ldots,x_T)\in \RR_+^T, \phantom{1} \sum_{t=1}^{T} x_t = N \right\}
\end{equation}

Let $\overline{g}$ be the real extension of $g$, defined on $\RR_+$. It is strictly increasing  on $\RR_+$, and such that $\overline{g}(0)=0$ and $\displaystyle\lim_{+ \infty} \overline{g} = 1$.
Let $\overline{v_t}(x_t)=\left[p_t - c_t\cdot\overline{g}\Big(\displaystyle\sum_{k=1}^{t} x_k\Big)\right] x_t$ \\
Let $\overline{f}$, from $\RR^T\rightarrow \RR$, such that $\overline{f}(x)=\displaystyle\sum_{t=1}^{T} \overline{v_t}(x_t)\Big)$ \\
We finally consider the following optimization problem:\\

\begin{equation}\mbox{UB}_1 = \displaystyle\max_{x \in \CC}\overline{f}(x) \label{pbCont}
\end{equation}
Obviously, problem (\ref{pbCont}) is non convex. So getting an upper bound of (\ref{pbMain0}), requires global solving, which, in general proves to be as hard as solving the initial problem. There are nonetheless several motivations to study problem (\ref{pbCont}). 
Firstly, as the continuous relaxation of problem (\ref{pbMain0}), a global maximum or an upper bound of problem (\ref{pbCont}), which we denote $\mbox{UB}_2$), and will discuss in more details in section XXX, does provide an upper bound of the original problem $(\mbox{OPT}\leqslant \mbox{UB}_1\leqslant \mbox{UB}_2)$.\\
Secondly, when $N \gg T$, discrete approximation is accurate enough, so that discrete and continuous modeling should yield close results. Indeed, we show continuous optimization techniques can be efficiently used to refine lower bounds of the initial Problem (\ref{pbMain0}).
\\

Our purpose is either to solve problem (\ref{pbMain0}) exactly, under a CPU time limit, or to provide a tight interval for the optimal value, based on  both discrete  and continuous optimization.  \\
In the remaining of the paper, we will assume $g$ and $\overline{g}$ are continuously differentiable. Then, problem (\ref{pbCont}) is also well defined as $\CC$ is compact (XXX proof in appendix) and $\overline{f}$ is continuous. For numerical experiments, we selected concave functions with different convergence speeds to infinity: $g(x) = 1 - \frac 1 {1+x}$, $g(x) = 1 - \frac 2 {1+\sqrt{1+x}}$ ou $g(x) = \frac 2 {\pi} \mbox{arctan}(x)$.\\
Concavity is equivalent to decreasing first order derivative, which makes sense for numerical experiments.\\
While we selected a few penalty functions for numerical experiments, any increasing positive function $h$, satisfying aforementioned regularity conditions is eligible. Indeed, we can define the corresponding function $g$ on $\RR_+$, by $g: x\mapsto \frac{h(x)-h(0)}{h(L_{\infty})-h(0)}$, for some real $L_{\infty}>N$, so that when $y_t$ goes to N, $g$ can be arbitrarily close to 1. Hence the pool of candidates for penalty function is quite large.\\
Lastly, we did not apply any filter to the admissibility set $\DD$  to exclude unrealistic solutions. For instance, the \textit{fire sale} $(M,0,\cdots,0)$, which liquidates the whole block in one shot at the first time step, is admissible, while it very seldomly is in practice. We are not concerned by lack of liquidity in the market and potential trading halt, due to exchange circuit-breakers, triggered upon a strong selling action at any time step. We assume optimal solutions to be practically feasible. In most cases, solutions stemming from instances considered in numerical experiments remain below the system limits for most blue chip company stock.  We did not however carry out any further analysis about it.

==> recap_cst_largeInstances_cpu_tab2.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
T&N&5&5&5&5&5&5&5           \\\hline
T&N&FS&US&ILS&LS&TS1&TS2&UB \\\hline
$10^1$&$10^7$&$<\epsilon$&$<\epsilon$&$<\epsilon$&600&19.21&5.7&$<\epsilon$         \\\hline
$10^1$&$10^8$&$<\epsilon$&$<\epsilon$&3.34&600&195.45&18.01&$<\epsilon$             \\\hline
$10^1$&$10^9$&$<\epsilon$&$<\epsilon$&38.33&60&DNC&DNC&$<\epsilon$    \\\hline
$10^2$&$10^6$&$<\epsilon$&$<\epsilon$&0.21&60&28.1&10.18&$<\epsilon$  \\\hline
$10^2$&$10^7$&$<\epsilon$&$<\epsilon$&0.29&600&1041.73&1011.34&$<\epsilon$          \\\hline
$10^2$&$10^8$&$<\epsilon$&$<\epsilon$&4.89&60&DNC&DNC&$<\epsilon$     \\\hline
$10^2$&$10^9$&$<\epsilon$&$<\epsilon$&39.34&60&DNC&DNC&$<\epsilon$    \\\hline
$10^3$&$10^6$&$<\epsilon$&$<\epsilon$&154.12&600&557.35&396.7&$<\epsilon$           \\\hline
$10^3$&$10^7$&$<\epsilon$&$<\epsilon$&257.41&600&DNC&DNC&$<\epsilon$  \\\hline
$10^3$&$10^8$&$<\epsilon$&$<\epsilon$&366.52&600&DNC&DNC&$<\epsilon$  \\\hline
$10^3$&$10^9$&$<\epsilon$&$<\epsilon$&648.6&600&DNC&DNC&$<\epsilon$   \\\hline
\end{tabular}

